COMET-ATOMIC 2020: On Symbolic and Neural Commonsense Knowledge Graphs

Recent years have brought about a renewed interest in commonsense representation and reasoning in the field of natural language understanding. The development of new commonsense knowledge graphs (CSKG) has been central to these advances as their diverse facts can be used and referenced by machine learning models for tackling new and challenging tasks. At the same time, there remain questions about the quality and coverage of these resources due to the massive scale required to comprehensively encompass general commonsense knowledge. In this work, we posit that manually constructed CSKGs will never achieve the coverage necessary to be applicable in all situations encountered by NLP agents. Therefore, we propose a new evaluation framework for testing the utility of KGs based on how effectively implicit knowledge representations can be learned from them. With this new goal, we propose ATOMIC 2020, a new CSKG of general-purpose commonsense knowledge containing knowledge that is not readily available in pretrained language models. We evaluate its properties in comparison with other leading CSKGs, performing the first large-scale pairwise study of commonsense knowledge resources. Next, we show that ATOMIC 2020 is better suited for training knowledge models that can generate accurate, representative knowledge for new, unseen entities and events. Finally, through human evaluation, we show that the few-shot performance of GPT-3 (175B parameters), while impressive, remains ~12 absolute points lower than a BART-based knowledge model trained on ATOMIC 2020 despite using over 430x fewer parameters.

==> addl_tables.tex <==

\begin{table*}[t]
  \centering
\begin{tabular}{lrrrrrrrr}
\toprule
                       &   B-1 &   B-2 &   B-3 &   B-4 &   METEOR &   ROUGE-L &   CIDEr &   BERTScore \\
\toprule
 GPT2-0shot-\atomicTT &    0.104 &    0.029 &    0.010 &    0.004 &    0.082 &     0.100 &   0.048 &        0.395 \\
 GPT2-0shot-\atomic &    0.085 &    0.030 &    0.012 &    0.005 &    0.081 &     0.090 &   0.047 &        0.386 \\
 GPT2-0shot-ConceptNet &    0.044 &    0.012 &    0.004 &    0.002 &    0.064 &     0.057 &   0.051 &        0.389 \\
 GPT2-0shot-TransOMCS  &    0.028 &    0.001 &    0.000 &    0.000 &    0.093 &     0.054 &   0.014 &        0.351 \\
 \midrule
 BART-\atomicTT       &    0.473 &    0.289 &    0.192 &    0.132 &    0.330 &     0.501 &   0.665 &        0.639 \\
 BART-\atomic       &    0.523 &    0.329 &    0.225 &    0.164 &    0.347 &     0.554 &   0.750 &        0.646 \\
 BART-ConceptNet       &    0.172 &    0.111 &    0.072 &    0.049 &    0.130 &     0.184 &   0.369 &        0.535 \\
 BART-TransOMCS        &    0.351 &    0.170 &    0.003 &    0.000 &    0.198 &     0.352 &   0.297 &        0.678 \\
 \midrule
 T5-3B-\atomicTT      &    0.513 &    0.342 &    0.245 &    0.187 &    0.359 &     0.517 &   0.769 &        0.645 \\
 T5-3B-\atomic      &    0.591 &    0.425 &    0.321 &    0.257 &    0.390 &     0.600 &   0.831 &        0.656 \\
 T5-3B-ConceptNet      &    0.258 &    0.189 &    0.139 &    0.098 &    0.213 &     0.326 &   0.866 &        0.598 \\
 T5-3B-TransOMCS       &    0.399 &    0.629 &    0.007 &    0.001 &    0.238 &     0.401 &   0.437 &        0.694 \\
 \midrule
 T5-11B-\atomicTT     &    0.496 &    0.329 &    0.235 &    0.178 &    0.356 &     0.510 &   0.737 &        0.641 \\
 T5-11B-\atomic     &    0.574 &    0.415 &    0.316 &    0.255 &    0.385 &     0.581 &   0.809 &        0.652 \\
 T5-11B-ConceptNet     &    0.230 &    0.167 &    0.123 &    0.095 &    0.184 &     0.260 &   0.669 &        0.571 \\
 T5-11B-TransOMCS      &    0.379 &    0.000 &    0.000 &    0.000 &    0.228 &     0.381 &   0.399 &        0.690 \\
\bottomrule
\end{tabular}
\caption{Greedy decoding, all relations, 5k sampled prefixes for each KG}
\end{table*}

\begin{table}[t]
  \centering
\begin{tabular}{lcc}
\hline
         &   BART-ATOMIC &   BART-ATOMIC2020 \\
\hline
 oEffect &         0.796 &             0.797 \\
 oReact  &         0.813 &             0.807 \\
 xWant   &         0.533 &             0.537 \\
 xNeed   &         0.555 &             0.543 \\
 xAttr   &         0.686 &             0.686 \\
 oWant   &         0.717 &             0.725 \\
 xReact  &         0.633 &             0.626 \\
 xEffect &         0.510 &             0.533 \\
 xIntent &         0.572 &             0.557 \\
 \hline
 all     &         0.643 &             0.643 \\
\hline
\end{tabular}
\caption{BERT scores of BART generations for all the prefixes shared between \atomic{} and \atomicTT{}, broken down per relation.}
\end{table}

\begin{table}[t]
  \centering
\begin{tabular}{lcc}
\hline
         &   T5-11B-ATOMIC &   T5-11B-ATOMIC2020 \\
\hline
 oEffect &           0.811 &               0.797 \\
 oReact  &           0.830 &               0.808 \\
 xWant   &           0.547 &               0.541 \\
 xNeed   &           0.571 &               0.535 \\
 xAttr   &           0.672 &               0.658 \\
 oWant   &           0.686 &               0.724 \\
 xReact  &           0.648 &               0.639 \\
 xEffect &           0.559 &               0.517 \\
 xIntent &           0.584 &               0.560 \\
 \hline
 all     &           0.655 &               0.639 \\
\hline
\end{tabular}
\caption{BERT scores of T5 generations for all the prefixes shared between \atomic{} and \atomicTT{}, broken down per relation.}
\end{table}

\begin{table*}[t]
  \centering
\begin{tabular}{lcc}
\hline
             &   BART-ConceptNet &   BART-ATOMIC2020 \\
\hline
 CapableOf   &             0.499 &             0.525 \\
 AtLocation  &             0.695 &             0.686 \\
 HasProperty &             0.535 &             0.447 \\
 Causes      &             0.640 &             0.688 \\
 NotDesires  &             0.492 &             0.561 \\
 \hline
 all         &             0.633 &             0.629 \\
\hline
\end{tabular}
\caption{BERT scores for all the prefixes shared between \conceptnet{}{} and \atomicTT{}, broken down per relation.}
\end{table*}

\begin{table*}[t]
  \centering
\begin{tabular}{lcccc}
\hline
         &   BART-ATOMIC-TESTALL &   BART-ATOMIC2020-TESTALL &   BART-ATOMIC-TESTALL &   BART-ATOMIC2020-TESTALL \\
\hline
 all     &                 0.766 &                     0.769 &                 0.650 &                     0.650 \\
 oEffect &                 1.633 &                     1.631 &                 0.795 &                     0.796 \\
 oReact  &                 1.381 &                     1.382 &                 0.806 &                     0.806 \\
 oWant   &                 1.321 &                     1.308 &                 0.720 &                     0.717 \\
 xAttr   &                 0.240 &                     0.238 &                 0.682 &                     0.684 \\
 xEffect &                 0.257 &                     0.279 &                 0.507 &                     0.512 \\
 xIntent &                 0.827 &                     0.843 &                 0.615 &                     0.614 \\
 xNeed   &                 0.523 &                     0.515 &                 0.532 &                     0.529 \\
 xReact  &                 0.312 &                     0.315 &                 0.654 &                     0.653 \\
 xWant   &                 0.400 &                     0.406 &                 0.537 &                     0.539 \\
\hline
\end{tabular}
\caption{CIDEr and BERT scores of BART generations for all the prefixes shared between \atomic{} and \atomicTT{} in the full test set, broken down per relation.}
\end{table*}

\begin{table*}[t]
  \centering
\begin{tabular}{lcccc}
\hline
             &   BART-ConceptNet-TESTALL &   BART-ATOMIC2020-TESTALL &   BART-ConceptNet-TESTALL &   BART-ATOMIC2020-TESTALL \\
\hline
 all         &                     0.389 &                     0.386 &                     0.577 &                     0.590 \\
 AtLocation  &                     0.529 &                     0.509 &                     0.636 &                     0.652 \\
 CapableOf   &                     0.223 &                     0.269 &                     0.500 &                     0.514 \\
 Causes      &                     0.203 &                     0.093 &                     0.570 &                     0.588 \\
 HasProperty &                     0.194 &                     0.215 &                     0.500 &                     0.499 \\
 NotDesires  &                     0.306 &                     0.272 &                     0.494 &                     0.524 \\
 Desires     &                     0.098 &                     0.000 &                     0.488 &                     0.507 \\
\hline
\end{tabular}
\caption{CIDEr and BERT scores of BART generations for all the prefixes shared between \conceptnet{} and \atomicTT{} in the full test set, broken down per relation.}
\end{table*}


\begin{table}[t]
  \centering
\begin{tabular}{lcc}
\hline
             &   ConceptNet &   ATOMIC2020 \\
\hline
 AtLocation  &                     0.636 &                     0.652 \\
 CapableOf   &                     0.500 &                     0.514 \\
 Causes      &                     0.570 &                     0.588 \\
 HasProperty &                     0.500 &                     0.499 \\
 NotDesires  &                     0.494 &                     0.524 \\
 Desires     &                     0.488 &                     0.507 \\
 \hline
 all         &                     0.577 &                     0.590 \\
\hline
\end{tabular}
\caption{BERT scores of BART generations for all the test prefixes shared between \conceptnet{} and \atomicTT{}, broken down per relation.}
\end{table}

\begin{table*}[t]
  \centering
\begin{tabular}{lcccccccc}
\toprule
                       &   B-1 &   B-2 &   B-3 &   B-4 &   METEOR &   ROUGE-L &   CIDEr &   BERTScore \\
\toprule
 GPT2-0shot-\atomicTT &    0.104 &    0.029 &    0.010 &    0.004 &    0.082 &     0.100 &   0.048 &        0.395 \\
 GPT2-0shot-\atomic     &    0.085 &    0.030 &    0.012 &    0.005 &    0.081 &     0.090 &   0.047 &        0.386 \\
 GPT2-0shot-ConceptNet &    0.044 &    0.012 &    0.004 &    0.002 &    0.064 &     0.057 &   0.051 &        0.389 \\
 GPT2-0shot-TransOMCS  &    0.028 &    0.001 &    0.000 &    0.000 &    0.093 &     0.054 &   0.014 &        0.351 \\
\midrule
 BART-\atomicTT       &    0.446 &    0.267 &    0.184 &    0.134 &    0.320 &     0.476 &   0.670 &        0.628 \\
 BART-\atomic           &    0.473 &    0.288 &    0.203 &    0.153 &    0.333 &     0.520 &   0.735 &        0.629 \\
 BART-ConceptNet       &    0.184 &    0.119 &    0.081 &    0.055 &    0.144 &     0.182 &   0.383 &        0.517 \\
 BART-TransOMCS        &    0.340 &    0.227 &    0.004 &    0.000 &    0.194 &     0.340 &   0.293 &        0.670 \\
\midrule
 T5-L-\atomicTT       &    0.104 &    0.051 &    0.026 &    0.014 &    0.159 &     0.121 &   0.014 &        0.384 \\
 T5-L-\atomic           &    0.087 &    0.039 &    0.018 &    0.009 &    0.155 &     0.125 &   0.030 &        0.369 \\
 T5-L-ConceptNet       &    0.041 &    0.017 &    0.007 &    0.003 &    0.064 &     0.048 &   0.022 &        0.372 \\
 T5-L-TransOMCS        &    0.001 &    0.000 &    0.000 &    0.000 &    0.001 &     0.001 &   0.000 &        0.331 \\
\midrule
 T5-3B-\atomicTT      &    0.387 &    0.186 &    0.106 &    0.068 &    0.279 &     0.456 &   0.590 &        0.626 \\
 T5-3B-ConceptNet      &    0.190 &    0.118 &    0.074 &    0.045 &    0.155 &     0.236 &   0.616 &        0.563 \\
 T5-3B-TransOMCS       &    0.315 &    0.238 &    0.004 &    0.000 &    0.190 &     0.316 &   0.322 &        0.686 \\
\midrule
 T5-11B-\atomicTT     &    0.399 &    0.202 &    0.116 &    0.072 &    0.282 &     0.459 &   0.603 &        0.630 \\
 T5-11B-ConceptNet     &    0.195 &    0.127 &    0.087 &    0.060 &    0.152 &     0.223 &   0.581 &        0.557 \\
 T5-11B-TransOMCS      &    0.268 &    0.000 &    0.000 &    0.000 &    0.169 &     0.269 &   0.275 &        0.679 \\
\bottomrule
\end{tabular}
\caption{All relations}
\end{table*}

\begin{table*}[t]
  \centering
\begin{tabular}{lrrrrrrrr}
\toprule
                       &   B-1 &   B-2 &   B-3 &   B-4 &   METEOR &   ROUGE-L &   CIDEr &   BERTScore \\
\toprule
 GPT2-0shot-ConceptNet &    0.154 &    0.065 &    0.000 &    0.000 &    0.132 &     0.142 &   0.079 &        0.392 \\
 GPT2-0shot-TransOMCS  &    0.000 &    0.000 &    0.000 &    0.000 &    0.000 &     0.000 &   0.000 &        0.346 \\
\midrule
 BART-ConceptNet       &    0.433 &    0.342 &    0.266 &    0.217 &    0.340 &     0.365 &   0.253 &        0.473 \\
 BART-TransOMCS        &    0.000 &    0.000 &    0.000 &    0.000 &    0.000 &     0.000 &   0.000 &        0.417 \\
\midrule
 T5-L-ConceptNet       &    0.149 &    0.067 &    0.028 &    0.011 &    0.184 &     0.124 &   0.013 &        0.383 \\
 T5-L-TransOMCS        &    0.000 &    0.000 &    0.000 &    0.000 &    0.000 &     0.000 &   0.000 &        0.244 \\
\midrule
 T5-3B-ConceptNet      &    0.345 &    0.233 &    0.146 &    0.000 &    0.245 &     0.316 &   0.367 &        0.513 \\
 T5-3B-TransOMCS       &    0.000 &    0.000 &    0.000 &    0.000 &    0.000 &     0.000 &   0.000 &        0.650 \\
\midrule
 T5-11B-ConceptNet     &    0.371 &    0.263 &    0.179 &    0.133 &    0.273 &     0.307 &   0.421 &        0.499 \\
 T5-11B-TransOMCS      &    0.000 &    0.000 &    0.000 &    0.000 &    0.000 &     0.000 &   0.000 &        0.634 \\
\midrule
\end{tabular}
\caption{HasPrerequisite}
\end{table*}

\begin{table*}[t]
  \centering
\begin{tabular}{lrrrrrrrr}
\toprule
                       &   B-1 &   B-2 &   B-3 &   B-4 &   METEOR &   ROUGE-L &   CIDEr &   BERTScore \\
\midrule
 GPT2-0shot-\atomicTT &    0.000 &    0.000 &    0.000 &    0.000 &    0.000 &     0.000 &   0.000 &        0.389 \\
 GPT2-0shot-ConceptNet &    0.124 &    0.033 &    0.000 &    0.000 &    0.094 &     0.117 &   0.037 &        0.387 \\
 GPT2-0shot-TransOMCS  &    0.012 &    0.000 &    0.000 &    0.000 &    0.048 &     0.015 &   0.001 &        0.365 \\
\midrule
 BART-\atomicTT       &    0.000 &    0.000 &    0.000 &    0.000 &    0.000 &     0.000 &   0.000 &        0.532 \\
 BART-ConceptNet       &    0.297 &    0.167 &    0.076 &    0.059 &    0.210 &     0.247 &   0.184 &        0.453 \\
 BART-TransOMCS        &    0.544 &    0.000 &    0.000 &    0.000 &    0.277 &     0.572 &   0.677 &        0.730 \\
\midrule
 T5-L-\atomicTT       &    0.000 &    0.000 &    0.000 &    0.000 &    0.000 &     0.000 &   0.000 &        0.350 \\
 T5-L-ConceptNet       &    0.121 &    0.053 &    0.026 &    0.011 &    0.124 &     0.092 &   0.017 &        0.366 \\
 T5-L-TransOMCS        &    0.000 &    0.000 &    0.000 &    0.000 &    0.000 &     0.000 &   0.000 &        0.351 \\
\midrule
 T5-3B-\atomicTT      &    0.059 &    0.000 &    0.000 &    0.000 &    0.056 &     0.111 &   0.278 &        0.616 \\
 T5-3B-ConceptNet      &    0.225 &    0.139 &    0.100 &    0.082 &    0.169 &     0.206 &   0.302 &        0.495 \\
 T5-3B-TransOMCS       &    0.302 &    0.000 &    0.000 &    0.000 &    0.193 &     0.325 &   0.323 &        0.690 \\
\midrule
 T5-11B-\atomicTT     &    0.067 &    0.000 &    0.000 &    0.000 &    0.069 &     0.037 &   0.093 &        0.644 \\
 T5-11B-ConceptNet     &    0.236 &    0.161 &    0.106 &    0.092 &    0.174 &     0.223 &   0.277 &        0.497 \\
 T5-11B-TransOMCS      &    0.139 &    0.000 &    0.000 &    0.000 &    0.091 &     0.152 &   0.137 &        0.657 \\
\midrule
\end{tabular}
\caption{Causes}
\end{table*}

\begin{table*}[t]
  \centering
\begin{tabular}{lrrrrrrrr}
\toprule
                       &   B-1 &   B-2 &   B-3 &   B-4 &   METEOR &   ROUGE-L &   CIDEr &   BERTScore \\
\midrule
 GPT2-0shot-\atomicTT &    0.202 &    0.052 &    0.022 &    0.000 &    0.131 &     0.155 &   0.031 &        0.360 \\
 GPT2-0shot-ConceptNet &    0.060 &    0.018 &    0.007 &    0.000 &    0.114 &     0.068 &   0.037 &        0.391 \\
 GPT2-0shot-TransOMCS  &    0.016 &    0.002 &    0.000 &    0.000 &    0.064 &     0.023 &   0.003 &        0.351 \\
 \midrule
 BART-\atomicTT       &    0.512 &    0.359 &    0.257 &    0.185 &    0.396 &     0.429 &   0.245 &        0.482 \\
 BART-ConceptNet       &    0.391 &    0.275 &    0.187 &    0.141 &    0.321 &     0.364 &   0.491 &        0.546 \\
 BART-TransOMCS        &    0.388 &    0.244 &    0.004 &    0.000 &    0.259 &     0.402 &   0.271 &        0.641 \\
 \midrule
 T5-L-\atomicTT       &    0.234 &    0.122 &    0.060 &    0.028 &    0.268 &     0.199 &   0.008 &        0.394 \\
 T5-L-ConceptNet       &    0.107 &    0.050 &    0.023 &    0.010 &    0.186 &     0.140 &   0.044 &        0.401 \\
 T5-L-TransOMCS        &    0.002 &    0.000 &    0.000 &    0.000 &    0.002 &     0.002 &   0.000 &        0.348 \\
 \midrule
 T5-3B-\atomicTT      &    0.370 &    0.209 &    0.126 &    0.000 &    0.286 &     0.308 &   0.139 &        0.483 \\
 T5-3B-ConceptNet      &    0.281 &    0.181 &    0.112 &    0.085 &    0.206 &     0.269 &   0.374 &        0.521 \\
 T5-3B-TransOMCS       &    0.334 &    0.356 &    0.005 &    0.001 &    0.225 &     0.341 &   0.295 &        0.677 \\
 \midrule
 T5-11B-\atomicTT     &    0.451 &    0.277 &    0.177 &    0.121 &    0.292 &     0.351 &   0.146 &        0.490 \\
 T5-11B-ConceptNet     &    0.335 &    0.218 &    0.170 &    0.137 &    0.226 &     0.312 &   0.404 &        0.534 \\
 T5-11B-TransOMCS      &    0.297 &    0.000 &    0.000 &    0.000 &    0.210 &     0.310 &   0.231 &        0.668 \\
\midrule
\end{tabular}
\caption{ObjectUse, UsedFor}
\end{table*}


\begin{table*}[t]
  \centering
\begin{tabular}{lrrrrrrrr}
\toprule
                   &   B-1 &   B-2 &   B-3 &   B-4 &   METEOR &   ROUGE-L &   CIDEr &   BERTScore \\
\midrule
 BART-\atomicTT &    0.473 &    0.289 &    0.192 &    0.132 &    0.330 &     0.501 &   0.665 &        0.639 \\
 BART-ConceptNet &    0.172 &    0.111 &    0.072 &    0.049 &    0.130 &     0.184 &   0.369 &        0.535 \\
 BART-TransOMCS  &    0.351 &    0.170 &    0.003 &    0.000 &    0.198 &     0.352 &   0.297 &        0.678 \\
 \midrule
 T5-3B-\atomicTT  &    0.513 &    0.342 &    0.245 &    0.187 &    0.359 &     0.517 &   0.769 &        0.645 \\
 T5-3B-ConceptNet  &    0.258 &    0.189 &    0.139 &    0.098 &    0.213 &     0.326 &   0.866 &        0.598 \\
 T5-3B-TransOMCS   &    0.399 &    0.629 &    0.007 &    0.001 &    0.238 &     0.401 &   0.437 &        0.694 \\
 \midrule
 T5-11B-\atomicTT &    0.496 &    0.329 &    0.235 &    0.178 &    0.356 &     0.510 &   0.737 &        0.641 \\
 T5-11B-ConceptNet &    0.230 &    0.167 &    0.123 &    0.095 &    0.184 &     0.260 &   0.669 &        0.571 \\
 T5-11B-TransOMCS  &    0.379 &    0.000 &    0.000 &    0.000 &    0.228 &     0.381 &   0.399 &        0.690 \\
\midrule
\end{tabular}
\caption{Greedy}
\end{table*}

% \begin{table}[]
% \begin{tabular}{lrrr}
% \toprule
% \textbf{Relation / Model}          & N   & \gptxl & \cometbart \\
% \midrule
% AtLocation  & 88  & 68.2     & 87.5  \\
% CapableOf   & 31  & 41.9     & 80.6  \\
% Causes      & 9   & 100.0    & 66.7  \\
% Desires     & 1   & 100.0    & 100.0  \\
% HasProperty & 24  & 50.0     & 75.0  \\
% HasSubEvent & 15  & 66.7     & 100.0  \\
% HinderedBy  & 378 & 1.3      & 85.4  \\
% MadeUpOf    & 19  & 47.4     & 78.9  \\
% NotDesires  & 1   & 0.0      & 0.0  \\
% ObjectUse   & 192 & 43.2     & 79.7  \\
% isAfter     & 432 & 29.2     & 90.5  \\
% isBefore    & 424 & 44.8     & 90.8  \\
% isFilledBy  & 129 & 7.0      & 89.1  \\
% oEffect     & 357 & 29.7     & 73.9  \\
% oReact      & 371 & 40.7     & 81.1  \\
% oWant       & 357 & 75.1     & 88.2  \\
% xAttr       & 355 & 30.7     & 92.1  \\
% xEffect     & 350 & 18.9     & 69.7  \\
% xIntent     & 349 & 28.9     & 75.9  \\
% xNeed       & 396 & 33.6     & 82.1  \\
% xReact      & 362 & 47.0     & 94.5  \\
% xWant       & 359 & 55.4     & 88.9  \\
% \bottomrule
% \end{tabular}
% \caption{Human - \atomicTT}
% \end{table}

% \begin{table}[]
% \begin{tabular}{lrrr}
% \toprule
% \textbf{Relation / Model}          & $N$   & \gptxl & \cometbart \\
% \midrule
% oEffect          & 524 & 31.7 & 70.4  \\
% oReact           & 553 & 42.3 & 80.7  \\
% oWant            & 522 & 72.6 & 89.7  \\
% xAttr            & 588 & 32.0 & 91.7  \\
% xEffect          & 608 & 21.1 & 71.5  \\
% xIntent          & 585 & 27.5 & 76.6  \\
% xNeed            & 549 & 29.3 & 84.0  \\
% xReact           & 551 & 41.9 & 94.7  \\
% xWant            & 520 & 51.7 & 89.6  \\
% \bottomrule
% \end{tabular}
% \caption{Human Evaluation Precision - \atomic}
% \end{table}

% \begin{table}[]
% \begin{tabular}{lrrr}
% \toprule
% \textbf{Relation / Model}          & $N$   & \gptxl & \cometbart \\
% \midrule
% AtLocation       & 511 & 68.1   & 85.7  \\
% CapableOf        & 625 & 50.9   & 74.9  \\
% Causes           & 99  & 63.6   & 80.8  \\
% CausesDesire     & 207 & 61.4   & 73.9  \\
% Desires          & 49  & 46.9   & 83.7  \\
% HasA             & 287 & 28.6   & 73.9  \\
% HasFirstSubevent & 36  & 33.3   & 61.1  \\
% HasLastSubevent  & 38  & 34.2   & 68.4  \\
% HasPrerequisite  & 80  & 78.8   & 86.3  \\
% HasProperty      & 587 & 46.5   & 71.0  \\
% HasSubevent      & 150 & 52.7   & 90.0  \\
% MadeOf           & 35  & 54.3   & 74.3  \\
% MotivatedByGoal  & 109 & 47.7   & 59.6  \\
% NotDesires       & 21  & 28.6   & 71.4  \\
% PartOf           & 104 & 58.7   & 49.0  \\
% ReceivesAction   & 357 & 35.6   & 72.3  \\
% UsedFor          & 241 & 46.1   & 79.7  \\
% \bottomrule
% \end{tabular}
% \caption{Human Evaluation Precision - \conceptnet}
% \end{table}

% \begin{table}[]
% \begin{tabular}{lrrr}
% \toprule
% \textbf{Relation / Model}          & $N$   & \gptxl & \cometbart \\
% \midrule
% AtLocation       & 507 & 49.7   & 30.6 \\
% CapableOf        & 812 & 31.5   & 7.9 \\
% Causes           & 61  & 37.7   & 4.9 \\
% CausesDesire     & 253 & 29.6   & 29.2 \\
% Desires          & 6   & 33.3   & 16.7 \\
% HasA             & 550 & 16.4   & 38.4 \\
% HasFirstSubevent & 29  & 17.2   & 3.4 \\
% HasLastSubevent  & 47  & 23.4   & 14.9 \\
% HasPrerequisite  & 1   & 100.0  & 0.0 \\
% HasProperty      & 410 & 32.4   & 47.3 \\
% HasSubevent      & 18  & 27.8   & 11.1 \\
% MadeOf           & 221 & 15.4   & 4.5 \\
% MotivatedByGoal  & 9   & 11.1   & 0.0 \\
% PartOf           & 138 & 50.0   & 34.1 \\
% ReceivesAction   & 785 & 22.7   & 21.0 \\
% UsedFor          & 547 & 22.9   & 20.5 \\
% \bottomrule
% \end{tabular}
% \caption{Human Evaluation Precision - \transomcs}
% \end{table}

==> tables/tab-new-relations.tex <==

% V1  (with entity/events on the size)
\begin{comment}
\begin{table}[t]
    \small
    \centering
    %\setlength\tabcolsep{3pt} 
    \begin{tabular}{p{1em}p{5em}clr}
    \toprule
    &\textbf{Head}  & \textbf{New Relation} & \textbf{Tail} & \textbf{Size}\\
    \midrule
    & \multirow{4}{*}{bread} & ObjectUse & \makecell[l]{make french toast;\\attracts ants} & $165590$\\
    \cmidrule{3-5}
    \multirow{7}{*}{\rotatebox[origin=c]{90}{ Entity-Related}}
    &  & AtLocation* & basket; pantry & $20221$\\
    \cmidrule{3-5}
    &  & MadeUpOf & dough; wheat  & $3345$\\
    \cmidrule{3-5}
    &  & HasProperty* & cooked; nice to eat & $5617$\\
    \cmidrule{2-5}
    & \multirow{3}{*}{baker} & CapableOf* & \makecell[l]{bake bread;\\coat cake with icing} & $7968$\\
    \cmidrule{3-5}
    && Desires* & quality ingredients & $2737$\\
    \cmidrule{3-5}
    && Not Desires* & bad yeast & $2838$\\
    \midrule
    &\multirow{6}{*}{\makecell{X runs out\\of steam}} & IsAfter & X exercises in the gym & $22453$\\
    \cmidrule{3-5}
    \multirow{7}{*}{\rotatebox[origin=c]{90}{Event-Related}}
    && IsBefore & X hits the showers & $23208$\\
    \cmidrule{3-5}
    && HinderedBy & drinks too much coffee & $106658$\\
    \cmidrule{3-5}
    && Causes & takes a break & $376$\\
    \cmidrule{3-5}
    && xReason & did not eat breakfast & $334$ \\
    \cmidrule{3-5}
    && HasSubEvent & become tired  & $12845$\\
    \cmidrule{2-5}
    & \makecell{X watches\\\_\_\_ anyway} & isFilledBy & the game; the TV & $33266$\\
    \bottomrule
    \end{tabular}
    \caption{New relations in \atomicTT{}. Relations that reflect semantically identical categories to \conceptnet{} is marked with asterisk (*).}
    \label{tab:atomic2020-newrelations}
\end{table}
\end{comment}

% V2  (with Entity/Events on top and sizes in K)
\begin{comment}
\begin{table}[t]
    \small
    \centering
    \setlength\tabcolsep{3pt} 
    \begin{tabular}{p{5em}p{6em}p{9.5em}r}
    \toprule
    \textbf{Head}  & \makecell[l]{\textbf{New}\\\textbf{Relation}} & \textbf{Tail} & \textbf{Size (K)}\\
    \midrule
    % \multirow{7}{*}{\rotatebox[origin=c]{90}{ Entity-Related}}
    \multicolumn{4}{l}{\textsc{Entity-Related}}\\
    \midrule
    \multirow{4}{*}{bread} & ObjectUse & \makecell[l]{make french toast;\\attracts ants} & $166.0$\\
    \cmidrule{2-4}
    & AtLocation* & basket; pantry & $20.0$\\
    \cmidrule{2-4}
    & MadeUpOf & dough; wheat  & $3.3$\\
    \cmidrule{2-4}
    & HasProperty* & cooked; nice to eat & $5.6$\\
    \midrule
    \multirow{3}{*}{baker} & CapableOf* & \makecell[l]{bake bread;\\coat cake with icing} & $8.0$\\
    \cmidrule{2-4}
    & Desires* & quality ingredients & $2.7$\\
    \cmidrule{2-4}
    & Not Desires* & bad yeast & $2.8$\\
    \midrule
    \midrule
    % \multirow{7}{*}{\rotatebox[origin=c]{90}{Event-Related}}
    \multicolumn{4}{l}{\textsc{Event-Related}}\\
    \midrule
    \multirow{6}{*}{\makecell{X runs out\\of steam}} & IsAfter & X exercises in the gym & $22.5$\\
    \cmidrule{2-4}
    & IsBefore & X hits the showers & $23.2$\\
    \cmidrule{2-4}
    & HinderedBy & drinks too much coffee & $106.7$\\
    \cmidrule{2-4}
    & Causes & takes a break & $0.4$\\
    \cmidrule{2-4}
    & xReason & did not eat breakfast & $0.3$ \\
    \cmidrule{2-4}
    & HasSubEvent & become tired  & $12.8$\\
    \midrule
    \makecell{X watches\\\_\_\_ anyway} & isFilledBy & the game; the TV & $33.3$\\
    \bottomrule
    \end{tabular}
    \caption{New relations in \atomicTT{} along with their size and illustrative examples. Relations that reflect semantically identical categories to \conceptnet{} is marked with asterisk (*).}
    \label{tab:atomic2020-newrelations}
\end{table}
\end{comment}

% V3, with full sizes
\begin{table}[t]
    \small
    \centering
    \setlength\tabcolsep{3pt} 
    \begin{tabular}{p{5em}p{6em}p{9.5em}r}
    \toprule
    \textbf{Head}  & \makecell[l]{\textbf{New}\\\textbf{Relation}} & \textbf{Tail} & \textbf{Size}\\
    \midrule
    % \multirow{7}{*}{\rotatebox[origin=c]{90}{ Entity-Related}}
    \multicolumn{4}{l}{\textsc{Entity-Related}}\\
    \midrule
    \multirow{4}{*}{bread} & ObjectUse & \makecell[l]{make french toast;\\attracts ants} & $165{,}590$\\
    \cmidrule{2-4}
    & AtLocation* & basket; pantry & $20{,}221$\\
    \cmidrule{2-4}
    & MadeUpOf & dough; wheat  & $3{,}345$\\
    \cmidrule{2-4}
    & HasProperty* & cooked; nice to eat & $5{,}617$\\
    \midrule
    \multirow{3}{*}{baker} & CapableOf* & \makecell[l]{bake bread;\\coat cake with icing} & $7{,}968$\\
    \cmidrule{2-4}
    & Desires* & quality ingredients & $2{,}737$\\
    \cmidrule{2-4}
    & Not Desires* & bad yeast & $2{,}838$\\
    \midrule
    \midrule
    % \multirow{7}{*}{\rotatebox[origin=c]{90}{Event-Related}}
    \multicolumn{4}{l}{\textsc{Event-Related}}\\
    \midrule
    \multirow{6}{*}{\makecell{X runs out\\of steam}} & IsAfter & X exercises in the gym & $22{,}453$\\
    \cmidrule{2-4}
    & IsBefore & X hits the showers & $23{,}208$\\
    \cmidrule{2-4}
    & HinderedBy & drinks too much coffee & $106{,}658$\\
    \cmidrule{2-4}
    & Causes & takes a break & $376$\\
    \cmidrule{2-4}
    & xReason & did not eat breakfast & $334$ \\
    \cmidrule{2-4}
    & HasSubEvent & become tired  & $12{,}845$\\
    \midrule
    \makecell{X watches\\\_\_\_ anyway} & isFilledBy & the game; the TV & $33{,}266$\\
    \bottomrule
    \end{tabular}
    \caption{New relations in \atomicTT{} along with their size and illustrative examples. Relations that reflect semantically identical categories to \conceptnet{} is marked with asterisk (*).}
    \label{tab:atomic2020-newrelations}
\end{table}


